Monitoring Dynamic Mobile Ad-Hoc Networks: A Fully Distributed Hybrid Architecture

The mobile ad-hoc networks (MANETs) represent a broad area of study and market interest. They provide a wide set of applications in multiple domains. In that context, the functional and non-functional monitoring of these networks is crucial. For that purpose, monitoring techniques have been deeply studied in wired networks using gossip-based or hierarchical-based approaches. However, when applied to a MANET, several problematics arise mainly due to the absence of a centralized administration, the inherent MANETs constraints and the nodes mobility. In this paper, we present a hybrid distributed monitoring architecture for mobile adhoc networks in context of mobility pattern. We get inspired of gossip-based and hierarchical-based algorithms for query dissemination and data aggregation. We define gossip-based mechanisms that help our virtual hierarchical topology to complete the data aggregation, and then ensure the stability and robustness of our approach in dynamic environments. Further, we propose a fully distributed monitoring protocol that ease the nodes communications. We evaluate our approach through a simulated testbed by using NS3 and Docker, and illustrate the efficiency of our mechanisms.

==> 03_methods/timeline.tex <==
\begin{figure}
\centering

\scalebox{0.95}{%

\begin{tikzpicture}[node distance=2cm,auto,>=stealth']
  \node[] (node0) {node0};
  \node[right = of node0] (node11) {node1.1};
  \node[right = of node11] (node21) {node2.1};
  \node[below of=node0, node distance=4cm] (node0_ground) {};
  \node[below of=node11, node distance=4cm] (node11_ground) {};
  \node[below of=node21, node distance=4cm] (node21_ground) {};
  %
  \draw (node21) -- (node21_ground);
  \draw (node11) -- (node11_ground);
  \draw (node0) -- (node0_ground);
  \draw[<-] ($(node11)!0.25!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node0)!0.25!(node0_ground)$);

  \draw[->] ($(node11)!0.40!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node0)!0.40!(node0_ground)$);
  \draw[->] ($(node11)!0.40!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node21)!0.40!(node21_ground)$);
  \draw[-] ($(node0)!0.40!(node0_ground)$) -- node[left,scale=0.7,midway]{acc(ACK\_IP)} ($(node0)!0.40!(node0_ground)$);

  \draw[-] ($(node21)!0.50!(node21_ground)$) -- node[right,scale=0.7,midway]{edgeNode()} ($(node21)!0.50!(node21_ground)$);

  \draw[->] ($(node21)!0.60!(node21_ground)$) -- node[above,scale=0.7,midway]{SND Aggregate} ($(node11)!0.60!(node11_ground)$);

  \draw[->] ($(node11)!0.75!(node11_ground)$) -- node[above,scale=0.7,midway]{SND AggregateACK} ($(node21)!0.75!(node21_ground)$);
  \draw[->] ($(node11)!0.75!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Aggregate} ($(node0)!0.75!(node0_ground)$);

  \draw[->] ($(node0)!0.90!(node0_ground)$) -- node[above,scale=0.7,midway]{SND AggregateACK} ($(node11)!0.90!(node11_ground)$);

  \draw[-] ($(node0)!0.95!(node0_ground)$) -- node[left,scale=0.7,midway]{done()} ($(node0)!0.95!(node0_ground)$);
\end{tikzpicture}

}

\caption{Timeline view of the events between node0, node11 and node21 in the example presented} \label{fig:timeline}
\end{figure}
